Memory-Efficient Expert Routing for Distributed MoE Training

As Mixture-of-Experts (MoE) models scale toward hundreds of experts and higher top-$k$ routing, memory efficiency in distributed training becomes a critical bottleneck. Peak memory is dominated by the MoE block, not attention: every intermediate buffer in the MoE dispatch pipeline is individually scaled by top-k routing. The standard all-to-all dispatcher sends all routed tokens in a single collective step, requiring the full top-$k$-expanded buffer to be constructed at once. In this work, we propose RelayMoE, a ring-based MoE execution model that computes locally as expert weights or tokens circulate, avoiding full top-$k$-expanded dispatch buffers. RelayMoE selects between expert and token routing according to communication volume and overlaps transfers with computation. The ring structure naturally supports memory-efficient MoE recomputation during backward: each hop reconstructs expert intermediates, uses them to compute gradients, and releases them before the next hop. The saved memory supports longer sequences and larger batches, or retains more attention activations to reduce attention recomputation and improve training throughput. We evaluate RelayMoE on 30B$-$57B production MoE models and varied expert configurations. In single-layer MoE experiments, RelayMoE achieves a $2\times$ average speedup over Megatron-LM. In full-model training under the same GPU memory budget, it improves throughput by up to $2.02\times$ and extends the largest tested trainable sequence length by up to $2.85\times$.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.16   Emergency release: fixes a typo in the code.

Version 2.15   Bug fixes.  Documentation updates
	       New journals: AILET, TAIS, TAISAP, ACMJDS

Version 2.14   Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> figures/table_qwen_config.tex <==

\begin{comment}
    
\begin{table}[t]
\centering
\caption{Model architecture of production MoE models used in evaluation.}
\label{tab:eval_models}
\small
\begin{tabular}{lcc}
\toprule
 & \textbf{Qwen3-30B} & \textbf{Qwen2-57B} \\
\midrule
Layers              & 48    & 28 \\
Hidden dim          & 2048  & 3584 \\
Expert FFN dim      & 768   & 2560 \\
Routed experts      & 128   & 64 \\
Shared experts      & --    & 8 \\
Top-$k$             & 8     & 8 \\
Total params        & 30.5B & 57.4B \\
Active params       & 3.3B  & 14B \\
\bottomrule
\end{tabular}
\end{table}
\end{comment}



\begin{table}[t]
\centering
\caption{Training configurations for production architectures.}
\label{tab:eval_config}
\small
\begin{tabular}{lcc}
\toprule
 & \textbf{Qwen3-30B-A3B} & \textbf{Qwen2-57B-A14B} \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{l}{\textit{Model architecture}} \\
Layers              & 48    & 28 \\
Hidden dimension    & 2048  & 3584 \\
Expert FFN          & 768   & 2560 \\
Experts (routed)    & 128   & 64 \\
Top-$k$             & 8     & 8 \\
Shared experts      & --    & 8 \\
Total params        & 30.5B & 57.4B \\
Active params       & 3.3B  & 14B \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{l}{\textit{Parallelism configuration}} \\
TP (with SP)        & 2     & 2 \\
CP                  & 4     & 4 \\
PP                  & 4     & 4 \\
EP                  & 8     & 8 \\
ETP                 & 1     & 1 \\
Total GPUs          & 32    & 32 \\
\midrule
\rowcolor{gray!15}
\multicolumn{3}{l}{\textit{Training configuration}} \\
Micro-batch         & 12    & 12 \\
Global batch        & 48    & 48 \\
Precision           & bf16  & bf16 \\
\bottomrule
\end{tabular}
\end{table}

==> text/design.tex <==
\section{Design}
\label{sec:design}

%\name replaces the dispatch-then-compute paradigm with ring-based local computation. Rather than gathering tokens at the expert's location, \name circulates expert weights or token activations through a ring of GPUs. At each hop, a GPU computes partial results using only the token-expert pairs present on that device, and these partial results accumulate as the ring progresses. At any point during execution, each GPU holds only the resident data and the in-flight partitions of the current and next hop. This bounds the intermediate memory to a fraction of what the all-to-all dispatch pipeline requires, eliminating the dependency on the top-k routing factor and the coexisting dispatch buffers.  Figure~\ref{fig:ring_moe} illustrates the execution model. We first describe ring-based dispatch and its forward and backward execution (Section~\ref{sec:local}), then explain adaptive routing between experts and tokens (Section~\ref{sec:adaptive}), memory-efficient MoE recomputation (Section~\ref{sec:saving_MoE_recompute}), and selective attention recomputation (Section~\ref{sec:adaptive_recompute}).

\name replaces the dispatch-then-compute paradigm with ring-based local computation. It circulates expert weights or token activations through a ring of GPUs and computes partial results using the token--expert pairs available at each hop. These partial results accumulate as the ring progresses, avoiding the full top-$k$-expanded dispatch buffers required by all-to-all. Figure~\ref{fig:ring_moe} illustrates the execution model. We first describe ring-based dispatch and its forward and backward execution (Section~\ref{sec:local}), then explain adaptive routing between experts and tokens (Section~\ref{sec:adaptive}), memory-efficient MoE recomputation (Section~\ref{sec:saving_MoE_recompute}), and selective attention recomputation (Section~\ref{sec:adaptive_recompute}).


\subsection{Ring-Based MoE Dispatch \textcolor{blue}{updated, will replace the figures.}}
\label{sec:local}


\name circulates data through the expert-parallel group in a ring instead of gathering all routed tokens in a single step (Figure~\ref{fig:ring_moe}).
Both the experts and the tokens are partitioned across the EP group: each rank hosts a subset of the experts, as in standard expert parallelism, and holds the tokens of its local batch.
The ring circulates one of the two, the expert weights or the token activations, one rank's partition at a time, while the other remains resident on its GPUs; choosing which to circulate, routing expert or routing token, is the subject of Section~\ref{sec:adaptive}.
At each hop, a GPU receives one circulating partition, the \emph{visiting partition}, from its ring neighbor via peer-to-peer communication, computes partial results from it and the resident data, accumulates them into the output, and forwards the partition to the next GPU.
After $N$ hops, every partition has visited every GPU, so each token has been processed by all of its assigned experts and the output activation is complete.

To illustrate, consider a forward hop using routing expert. The GPU receives a set of visiting experts from its neighbor. It checks the routing map to find which local tokens selected any of the visiting experts. For matching pairs, it locally permutes the relevant tokens, executes the expert GEMM, weights the outputs by the router probabilities, and adds the results to the running output activation. Tokens that did not select any visiting expert are simply skipped. This selective computation ensures that no redundant work is performed at any hop.

The backward pass follows the same ring structure. At each hop, the GPU recomputes the forward activations using the visiting expert and local tokens, then computes partial gradients with respect to both the token activations and the expert weights. The token activation gradients are accumulated locally across hops. The expert weight gradients are collected via in-place addition to a circulating gradient buffer that travels alongside the expert weights through the ring, as detailed in Section~\ref{sec:overlap}.

\name is mathematically equivalent to all-to-all dispatch. Each token-expert pair computes the same GEMM with the same weights and the same router probabilities. The only difference is the execution order: all-to-all gathers all pairs at the destination GPU before computing, while \name accumulates partial outputs incrementally across hops. 
%Because tokens remain on their local GPU throughout execution, no top-k-expanded dispatch buffers are created. At any point during a forward hop, the GPU holds only its local token activations, the visiting experts, and the partial output being accumulated. This eliminates both compounding factors identified in Section~\ref{sec:motivation}: the per-buffer top-k expansion and the coexistence of multiple large intermediate activations in the dispatch pipeline.



At any point during execution, each GPU holds only its local data and
the in-flight partitions of the current and next hop, the intermediate GEMM results. The top-k-expanded dispatch buffers from Figure~\ref{fig:m2} are eliminated entirely: \name does not permute tokens for non-local experts, does not materialize top-k copies of any token, never gathers top-k-expanded activations at any GPU, and never constructs a top-k-expanded buffer during combine. Figure~\ref{fig:m3} shows the resulting memory profile under the same training configuration as Figure~\ref{fig:m1}: the MoE spikes are eliminated and peak memory is reduced by 13.9 GB. Figure~\ref{fig:m4} zooms into a single layer, confirming that the 2.6 GB dispatch buffers from Figure~\ref{fig:m2} no longer appear in either forward or backward passes. The peak memory of \name is therefore bounded by the local data plus a single visiting partition, eliminating the dependency on the top-k routing factor and the coexisting dispatch buffers identified in Section~\ref{sec:motivation}.


%ring-moe-flat.pdf
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/eurosys_memory_gain_via_ring_221287b3.pdf}
    \caption{Memory profile under \name with the same configuration as Figure~\ref{fig:m1}. Peak memory is reduced by 13.9 GB; MoE spikes are eliminated. }
    \label{fig:m3}
    %\vspace{-20pt}
\end{figure}

%ring-moe-flat-zoomin.pdf
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth,]{figures/eurosys_forward_backward_221287b3.pdf}
    \caption{Single-layer memory profile under \name.  The 2.6 GB coexisting dispatch buffers from Figure~\ref{fig:m2} are eliminated. MoE forward and backward now show small bumps from local expert computation rather than dispatch buffers.}
    \label{fig:m4}
\end{figure}




This design also eliminates the need for token dropping and capacity-factor padding. In all-to-all dispatch, routing imbalance causes some GPUs to receive disproportionately many tokens, requiring capacity factors to bound the receive buffer or token dropping to discard excess tokens. In \name, each GPU processes only its fixed local tokens at every hop, regardless of how the routing map distributes token-expert assignments across the EP group. Memory consumption is balanced across ranks by construction. For architectures with shared experts such as Qwen2-MoE, the shared experts are computed separately outside the ring, as they are replicated on every GPU and do not require cross-GPU communication.







\begin{comment}
    
The main motivating part of our design is to avoid materializing the aforementioned large intermediate buffers during dispatch. As long as we are dispatching for all possible computation in one single step, the design will require materializing top-k scaled memory overheads. The top-k not only creates a large buffer, but also, at the same time, scales the necessary communication by top-k times. Ring-MoE design achieves performance gains by avoiding both of them. First of all, Ring-MoE uses the ranks participating in expert parallel groups as hops to route through and compute locally, at the same time accumulating the necessary activations, gradients, etc. as it moves. MoE block is preceded by an attention block, so it receives already split activations, which mostly will choose non-local experts. So, the way Ring-MoE makes this data available to its respective rank for computation is by the movement of the necessary buffer via the full ring network once. This makes sure each rank gets to do the necessary computation as it would have done similarly with all-to-all/all-gather variation, but without having those extra buffers. There are 2 kinds of data that Ring-MoE moves: one is activation, the other is expert weights or gradients. Ring-MoE keeps one stationary, but moves the other one. All participating ranks receive some data and send out some data in peer-to-peer to neighboring hops. This process is further supported by how the MoE is computed. Each rank has a routing-map that is used to decide the top-k expert selection by each token. As we route the experts, these routing maps give Ring-MoE the capacity to determine if, in the current stage, we have the pair of a particular token, and an expert combination selected by the routing-map. If so, only then do we compute. This is exactly the computation done in all-to-all/all-gather, but with the added benefit of never materializing those large buffers. These extra buffer savings can significantly help the highest achievable performance during training. \\
The second direct benefit of this design is reduced communication volume. With the top-k scaling now gone, Ring-MoE's individual communication from hop to hop is much lower in volume. Even though in a ring with $N$ hops, we need $N$ computation stages, and $N$ communications per rank, having a lower amount of data to transfer can directly benefit the runtime, even without using the extra buffer for larger batches or sequences. We will further discuss that in the evaluation section.\\
The required communication volume gives Ring-MoE some more design flexibility. Most state-of-the-art systems prefer all-to-all or all-gather for dispatch, and the communication volume is always dependent on activation sizes. Another way is to move the experts, which is rarely done in current state-of-the-art systems. But all these support only one of the options; this is suboptimal. Apart from reducing the buffer and communication volume, Ring-MoE can choose the best possible option between routing tokens or experts. This allows further flexibility. Based on the token size and expert parameter count, Ring-MoE can adaptively choose which particular data to route and what to keep stationary during the ring-based computation. Compared to all-to-all forward, Ring-MoE does not introduce any new type of additional computation. In fact, it smartly computes the full thing in steps, without adding much computational overhead. The memory scaling always remains limited to activation sizes and experts. This frees up the memory, which can be further used to increase recompute, batch-size, or sequence length. In the backward, the computation again uses localized permutation per rank based on the routing-map, and performs the computation in a streaming pipeline. \\
An additional beneficial feature of Ring-MoE dispatch is automatic memory balancing. It is tied to load-balancing in overall. Capacity factor and padding are frequently used to make sure the load is balanced. Specially capacity factor with token dropping allows for avoiding one expert parallel rank getting too many tokens. In Ring-MoE, a rank receives activations of shape $[batch, seqlen/(CP*SP)]$ if both context parallelism and sequence parallelism are applied, assuming both are applied. It does not matter even if a rank gets a disproportionate amount of tokens; it only gets to compute a fixed amount of tokens, as the experts are kept moving in a ring. So, Ring-MoE can not have a larger memory peak in any rank, no matter how disproportionately a rank is picked during top-k selection. This can also indirectly help with overall load-balancing. Currently, it supports all of these variants.\\
Further, we want to point out that our Ring-MoE design can work without any special hardware requirements, as this design can work on any hardware that would support traditional all-to-all/all-gather MoE. In a later discussion, we show Ring-MoE can offer memory savings compared to most recent hardware-specific dispatchers, such as DeepEP. It can work with all common variants of data parallelism, pipeline parallelism, context parallelism, megatron-style sequence parallelism, virtual parallelism, etc.



\textcolor{red}{(we need to discuss a little about the figure.)}\\

Ring-MoE provides an easy estimate to pick between expert-routing or token-routing. Ring-MoE design also tries to optimize its own design space to achieve the best possible performance. In the following ~\ref{sec:adaptive}, we will introduce adaptive routing of Ring-MoE.
\end{comment}


\subsection{Overlapping Communication and Computation \textcolor{blue}{updated}} 
\label{sec:overlap}

%tripple ring orchestration image

%\begin{figure}[H]
%    \centering
%    \includegraphics[width=\linewidth ]{figures/Ring_MoE_3_ring_syncronization_for_backward_pass.pdf}
%    \caption{Triple-ring orchestration for two consecutive backward hops with routing expert. Three concurrent operations overlap at each hop: expert weight prefetch (top), local gradient computation (middle), and weight gradient transfer (bottom). Gradient reduction and post-processing execute sequentially between hops.}
%    \label{fig:async_ring}
%\end{figure}
% \textcolor{red}{The figure need to improved. distinguish between compute, communication, etc, Show different streams. }

\name converts a single all-to-all collective into N sequential peer-to-peer hops. While this eliminates both the top-k-expanded activations and the coexisting dispatch buffers in all-to-all dispatcher, it introduces N rounds of communication per MoE layer. Without careful overlap, this would make \name %significantly 
slower than all-to-all dispatch, negating the memory benefits. Overlapping communication with computation at each hop is therefore critical to making ring-based dispatch practical. In the forward pass, this requires overlapping two concurrent flows: local computation and weight transfer. In the backward pass, an additional gradient transfer flow must also be overlapped, which \name organizes as double-ring orchestration. We describe \name with expert routing strategies below.
%using routing expert as an example (Figure~\ref{fig:async_ring});
Routing token follows the same principle, with token activations and routing metadata circulating in place of expert weights and gradients.

In the forward pass, the overlap is straightforward. While a GPU computes using the currently visiting expert and its local tokens, it simultaneously prefetches the next expert's weights from its neighbor via asynchronous P2P communication. By the time the current hop's computation finishes, the next expert is already available locally, allowing computation to proceed without stalling. This overlaps communication with computation at each hop, reducing the per-hop time from the sum of computation and transfer to the maximum of the two, as shown in Figure ~\ref{fig:recompute_MoE_saving}.



The backward pass is more challenging because three distinct data flows must operate with maximum overlap at each hop. %concurrently (yes for 3 ring, no for 2 ring)
\name organizes these as two concurrent rings. %(Figure~\ref{fig:async_ring}):
\textbf{Ring 1: Local gradient computation.} Using the visiting expert and local tokens, the GPU first recomputes the forward activations (Section~\ref{sec:saving_MoE_recompute}), then computes the partial gradient with respect to local tokens. This is the core computation at each hop and provides the time window for the other two rings to transfer data.
\textbf{Ring 2: Merged Communication Ring} While computation proceeds on the current hop's expert, \name asynchronously prefetches the next hop's expert weights from the neighboring GPU, identical to the forward overlap strategy.
%\textbf{Ring 3: Weight gradient transfer.} 
For weight gradient movement, the accumulated gradient is combined with the weight prefetch and sent in a single communication. The weight gradient buffer for each visiting expert circulates through the ring alongside the expert weights,
%one step behind. (saying one step behind may confuse readers)
The key observation enabling this ring is that partial gradients at each hop are independent: a GPU can compute its local partial weight gradient without waiting for the gradient buffer from the previous hop. After local gradient computation completes, the GPU synchronizes with the incoming accumulated gradient buffer, adds its local partial gradient in-place, and asynchronously forwards the updated buffer to the next GPU.
These two rings overlap with each other: while Ring 1 computes, Ring 2 moves experts and gradients at sync. %The recomputation step in Ring 2 provides additional computation time compared to the forward pass, giving Rings 1 and 3 more time to complete their transfers. 
If the gradient buffer from Ring 2 has not arrived when Ring 1 finishes, the GPU stalls briefly until it does. With merged-ring orchestration, the per-hop backward time reduces from the sum of all four operations to the maximum of local computation and communication, plus a small synchronization and reduction step. For computation, \name can adopt optimized GEMM kernels such as GroupedGEMM to gain computational speedups.






%%We further improve the design of Ring-MoE by enabling communication and computation overlapping in the forward and backward. During both forward and backward each hop moves the experts or the token based on adaptive routing choice. We start asynchronous sending of the necessary data for the next hop, at the same time receiving data for the previous hop, while computing for the current hop. So, Ring-MoE has already started collecting or sending data for the next hop during current steps calculation. For expert-routing and token-routing, we prefetch experts and activations, respectively in forward, and in backward. Additionally, we improve the expert-routing backward pass even more, by asynchronously moving the partially collected gradients. Gradient buffers are costly to move in a serialized manner, because of its size. Ring-MoE carefully splits the gradient calculation in a such a way that the buffer movement can be also overlapped. This reduces the overlall runtime, as we show in our evaluation section in Fig. ~\ref{fig:timing_breakdwon}. Gradients of experts are dependent on token activations. But as tokens are statically placed in each GPU, and Ring-MoE is routing the experts during backward,  we propose using a gradient accumulator. Graident accumulator keeps adding up the partial gradients of each experts, also keeps moving through the ring. Each expert only gets a partial gradient value from the currently available tokens in the local hop, and then moves to the other hops. So, as soon as during a backward hop, local partial gradients are computed for an expert, we add them to the running gradient accumulator for that expert, and asynchronously start moving this accumulator in the next hop. This accumulator is the buffer that is actually carrying the gradients. The most important factor is that we do not need the accumulated gradients of any previous gradient calculations to calculate the partial gradients of locally available experts at the current hop. So, Ring-MoE waits until the partial gradient calculation is over, and keep receiving the accumulator buffer from previous hop. Only after the partial gradient is calculated, Ring-MoE performs a synchronization to make sure to have the recent gradient accumulator. Then Ring-MoE perform a simple reduction of already accumulated gradients and local partial gradients. Fig. \ref{fig:async_ring}. shows the overlapping of weight prefetch, gradient buffer transfer, and partial gradient calculation overlapping for 2 continuous hops. This is equivalent to having 3 rings running parallely, and Ring-MoE achives optimal backward performance by using this tripple ring orchestration. Ring-MoE design also includes common optimizations such as avoiding small P2P transfers, memory coalescing etc. 


\subsection{Adaptive Routing: Experts vs Tokens \textcolor{blue}{updated}}
\label{sec:adaptive}

\name can circulate either expert weights or token activations through the ring while the other remains resident on each GPU. Both modes produce identical results (Section~\ref{sec:local}), but they differ in communication volume.
Table~\ref{tab:routing} compares the two modes. With routing expert, expert weights circulate while tokens remain resident. With routing token, token activations and routing metadata circulate while experts remain resident, analogous to how Ring Attention circulates KV blocks for attention computation. The two modes are symmetric: one keeps tokens stationary and moves experts, the other keeps experts stationary and moves tokens.


Considering expert parallelism alone, the comparison involves two factors: per-hop communication volume and per-GPU resident memory (both modes require the same N hops). Routing expert communicates $E_{\text{local}} \times W$
per hop but keeps all local tokens $B \times S \times H$ resident. Routing token communicates $B \times S \times (H + M)$ per hop but keeps all local expert $E_{\text{local}} \times W$ resident. Routing expert is preferred when token activations are large relative to expert weights: the communication volume is smaller and the tokens, which would be expensive to move, remain stationary. Routing token is preferred when expert weights are large relative to token activations: the communication volume is smaller and the large expert weights remain stationary. \name evaluates both volumes from the model configuration and parallelism settings at the start of training and selects the mode with lower per-hop communication volume.

In distributed MoE training, EP typically works alongside other parallelism dimensions that further adjust both resident memory and communication volume. Sequence parallelism (SP) and context parallelism (CP) partition the sequence dimension, reducing tokens per GPU to $B \times S / (\text{SP} \times \text{CP})$. Expert tensor parallelism (ETP), splits each expert's weight matrices across GPUs, reducing per-expert weight size to   $W / \text{ETP}$. 
 MoE Parallel Folding~\cite{moeparallelfolding2025} makes \text{ETP} independent of the attention-layer \text{TP} parallelism. 
Both adjustments apply to both modes, as shown in the second section of Table~\ref{tab:routing}. Because these adjustments can shift the balance in either direction, the optimal mode depends on the full training configuration rather than the model architecture alone. For example, a model with many experts may favor routing expert under high ETP (which shrinks expert volume) but routing token under low ETP. \name evaluates both volumes at training start using the full configuration and selects the mode with lower per-hop communication.

MoE model architecture trends make this ring-based dispatch increasingly consequential. As shown in Table~\ref{tab:trend}, frontier MoE models have grown from 8 experts (Mixtral) to several hundred (Qwen3.5, Kimi K2), while EP degrees in practice remain bounded by hardware (typically 8--16). The number of experts per GPU $E/EP$ increase significantly, making routing expert transfer progressively larger volumes of expert weights at each hop. Routing token, which scales with tokens per GPU rather than expert count, becomes increasingly preferable for fine-grained MoE architectures.


\input figures/routing


The physical topology of the ring also matters. When EP spans multiple nodes, cross-node hops use inter-node links (e.g., RDMA) with substantially lower bandwidth than intra-node NVLink. All-to-all dispatchers address this through hierarchical algorithms and optimized kernels such as Tutel and DeepEP that pipeline cross-node transfers. \name's ring structure instead serializes communication into P2P hops, which creates opportunities to overlap each hop's transfer with local computation (Section~\ref{sec:overlap}), but requires careful scheduling to avoid underutilizing bandwidth on the fast intra-node hops. In practice, \name complements rather than replaces optimized all-to-all: it reduces peak memory regardless of topology, and its per-hop overlap is effective on both intra-node and cross-node configurations. We show extensive scaling studies to show the pure MoE-layer latency gains \name produces compared to all-to-all, Tutel, and FasterMoE.



\begin{comment}

Ring-MoE provides 2 different modes for routing: (i) routing experts, and (ii) routing tokens. In both forward and backward, the preceding or succeeding attention part provides the MoE block with either activations, or activation gradients in backward. Both routing experts and routing tokens provide a similar buffer saving, mentioned earlier. The choice is mostly about performance gains. What we have noticed, for most of the latest models, routing the experts is a better choice, as the trained tokens per iteration are often massive, and the volume of it is higher than expert volumes. But our observations show that it is possible that sometimes Ring-MoE with a routing token would reduce the necessary communication volume to route through an expert parallel group compared to routing experts. Both routing experts and routing tokens are computationally similar in forward and backward terms of FLOPs. But the movement of data is different, and the opportunity for overlapping in token routing is limited. 

%So, in this regard, we provide the following estimations to pick one dispatcher for optimal performance while both give similar memory gains.



%%%%%%%
\textbf{Routing Experts.} For expert routing, the cost can be approximated by the following.

\begin{align}
C_{of}, C_{ob} &=\frac{(N-1)EW}{B_e}\\
T_{\mathrm{expert}}
& \approx
\max\!\left(
C_{of},
T_{\mathrm{f}}
\right)
+\max\!\left(
C_{ob},
T_{\mathrm{b}}
\right)
+\frac{NEW}{B_e}
\end{align}

Where $W$ is the single expert size, $E$ experts per GPU. $(N-1)$ comes from the number of hops required for moving the expert weight buffer forward and backward. Ring-MoE also have to move the expert gradients $(N)$ times in backward to put it into its original GPU rank. $C_{of}, C_{ob}$ are the overlapped expert buffer movement time. $B_{e}$ is the communication bandwidth. %$\alpha_e$ is the overhead.
$T_{f}$ and $T_{b}$ are the computation times for forward and backward, which would be overlapped by routing the expert weights due to gradient and weight overlapping. We can further simplify this to a communication-only consideration for approximation:

\begin{align}
T_{\mathrm{expert}} &\approx  \frac{(3N-2)EW}{B_e}
\end{align}

\textbf{Routing Tokens.}
For routing tokens, Ring-MoE has to move the token activations, the intermediate activations after local expert computations. Along with that, moving the routing map and probability matrix, which are fixed costs. 

\begin{align}
C_{oft}, C_{obt}&=\frac{(N-1)(2T+R+P)}{B_{t}}\\
T_{\mathrm{token}}
\approx
&\max\!\left(
C_{oft},
T_{\mathrm{f}}
\right)
+\max\!\left(
C_{obt},
T_{\mathrm{b}}
\right)
+\frac{N(T+P)}{B_t}
\end{align}
Here, $T$ is the token activation size. In forward and backward, we need to move token activations and their intermediate activations after computing with experts. These $2T$ activations are moved $(N-1)$ hops both for forward and backward in overlap with computation. Additionally, the routing map sized $R$, and the routing probabilities $P$ are also moved. Assuming communication time will dominate, this can be simplified to the following:
\begin{align}
T_{\mathrm{token}} &\approx \frac{N(5T+2R+3P)}{B_t}
\end{align}
If $T_{token}>T_{expert}$, Ring-MoE prefers to route experts, rather than tokens, for the best possible runtime performance. One key difference between routing experts and routing tokens is that communication remains static for expert routing, which is not the case for token routing. Ring-MoE with a routing expert can provide the best possible overlapping, while this is limited for routing tokens.\\
\end{comment}







\subsection{Zero-Communication MoE Recomputation \textcolor{blue}{updated}}
\label{sec:saving_MoE_recompute}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/recompute_saving.pdf}
    \caption{RingMoE can use a single-ring collective in the backward pass for its necessary MoE recomputation. For \texttt{EP}=4: \texttt{h0}, \texttt{h1}, .. are hops in ring collectives. \texttt{R} is each hops required activation recompute. }
    \label{fig:recompute_MoE_saving}
    %\vspace{-20pt}
\end{figure}

Activation recomputation~\cite{chen2016training} is widely used in large-scale training to reduce peak memory by discarding intermediate activations during forward and recomputing them during backward. In standard all-to-all dispatch, MoE activations are top-k expanded and consume significant memory, making recomputation a necessity despite its computational overhead. Recomputation works by caching the necessary inputs and layer/sublayer information. Then replayed during backward to generate the intermediate activations. Without this for \texttt{N} layers, all of its intermediate activations have to be stored, making large model training impossible. The mechanism of doing it is similar across all kinds of MoE implementations. Figure ~\ref{fig:recompute_MoE_saving} shows the all-to-all dispatcher as an example with recomputation on, requiring 2 more additional collectives to replay the forward MoE computation during backward pass. This is necessary to generate  intermediate activations for gradient calculations. The process is repeated for each MoE-layer that is recomputed. \\
But in \name during backward pass, even with recompute on, it is not required to replay the forward MoE layer again to recompute the forward's activations. This allows to save 1 full ring communication across \texttt{EP} group.
In \name, MoE recomputation is essentially free:
during backward, experts must circulate through the ring to
compute weight and activation gradients. At each hop, both
the local tokens and the visiting expert are already present
on the GPU. Re-executing the local forward GEMM adds
only local computation that is fully overlapped by the ring
communication that must happen regardless.
%This is possible because during backward pass ring-collective, each hop contains all the necessary information exactly in place for intermediate activations to be recomputed in place, before its gradient calculations. 
This allows \name to fully gain all the benefits of recompute without adding any extra collective. Figure ~\ref{fig:recompute_saving} shows for \name, during backward: each hops recompute \texttt{(R)}  being done in place. \name produces exactly the same results without any extra collectives that is otherwise mandatory for other MoE dispatchers, gaining system performance. Not only that, the computation and communication are overlapped in this design also. \\
Saving MoE forward activations is not preferred because  storing intermediate results from each of the N hops per layer, would consume GPU memory without eliminating any meaningful overhead.

%In both all-to-all and \name, MoE layers should remain recomputed, but for different reasons. In all-to-all dispatch, MoE activations are top-k expanded and too large to keep in memory. In \name, MoE recomputation is essentially free: during backward, experts must circulate through the ring to compute weight and activation gradients. At each hop, both the local tokens and the visiting expert are already present on the GPU. Re-executing the local forward GEMM adds only local computation that is fully overlapped by the ring communication that must happen regardless. 
%Saving MoE forward activations would instead require storing intermediate results from each of the N hops per layer, consuming memory without eliminating any meaningful overhead.


%\textcolor{red}{incorrect paragraph}

\subsection{Adaptive Recomputation \textcolor{blue}{updated}}
\label{sec:adaptive_recompute}

\name significantly reduces MoE peak memory, leaving GPU memory unused under full recomputation. \name exploits this extra memory by selectively disabling recomputation to improve training throughput.

With MoE layers recomputed, \name uses the extra memory to selectively disable attention recomputation layers. %( attention recomputation [we do not separate out attention parts, although we may be can do it].) 
Each attention layer $i$ has several recomputation options $j$, each with a memory cost $m_{i,j}$ to save its activations, and a compute saving $c_{i,j}$ from not re-executing the corresponding operations during backward. Both can be estimated from the model configuration and parallelism settings. 
Taking grouped-query attention with FlashAttention as an example, the memory cost $m_{i,j}$ per transformer block includes the query, key, value, and output tensors, whose sizes depend on the micro-batch size, local sequence length, number of attention heads, and head dimension. The recompute cost $c_{i,j}$ is proportional to the attention FLOPs, which depends on the sequence length and attention type (e.g., full attention vs sliding window attention in hybrid architectures such as Qwen3.5). Under the memory constraint $M_{\text{GPU}}$ - $M_{\text{peak}}$, where $M_{\text{GPU}}$ is GPU memory capacity and $M_{\text{peak}}$ is Ring-MoE's peak memory under full recomputation. \name ranks all options by their compute-per-memory ratio $c_{i,j}/m_{i,j}$ and greedily selects options until the memory budget is exhausted. This selection requires only sorting over the set of layer-option pairs, which is linear in the number of layers and adds negligible overhead. This selection is computed once at the start of training and applied throughout.

%% ATC submission paragraph
%Each attention layer $i$ has several recomputation options $j$, each with a memory cost $m_{i,j}$ to save its activations, and a compute saving $c_{i,j}$ from not re-executing the corresponding operations during backward. Both can be estimated from the model configuration and parallelism settings. 
%Taking grouped-query attention with FlashAttention as an example, the memory cost $m_{i,j}$ per transformer block includes the query, key, value, and output tensors, whose sizes depend on the micro-batch size, local sequence length, number of attention heads, and head dimension. The recompute cost $c_{i,j}$ is proportional to the attention FLOPs, which depends on the sequence length and attention type (e.g., full attention vs sliding window attention in hybrid architectures such as Qwen3.5). Under the memory constraint $M_{\text{GPU}}$ - $M_{\text{peak}}$, where $M_{\text{GPU}}$ is GPU memory capacity and $M_{\text{peak}}$ is Ring-MoE's peak memory under full recomputation. \name ranks all options by their compute-per-memory ratio $c_{i,j}/m_{i,j}$ and greedily selects options until the memory budget is exhausted. This selection requires only sorting over the set of layer-option pairs, which is linear in the number of layers and adds negligible overhead. This selection is computed once at the start of training and applied throughout.

==> text/draft_old.tex <==

\section{Design}
to address memory issues on any platform, Ring-MoE introduces .... for sparse models with varied expert counts, and top-k routing.
we provide the overview in fiugre 1.. we propose first.., second .., third... (what we leverage? and what does our solution provide? what we reduced? what did we solve? what we remove?)
(deepseek has 256 experts with topk=8). We should have subsections of mentioned proposals

\begin{itemize}
    \item Ring P2P Memory Reduction
    \begin{itemize}
        \item how ring requires much less memory to for MoE block
    \end{itemize}
    \item Local Permute \& Expert Selection
    \item Concurrent Compute with Local Experts
    \item Expert Routing/activation Routing
    \begin{itemize}
        \item expert routing
        \item token routing
        \item some math for selection
    \end{itemize}
    \item Recompute Friendly Design (does not add extra communication for recompute)\\

\subsection{Memory Efficient MoE-Block}
some part will belong to motivation.\\
The most essential part of Ring-MoE design is to reduce the intermediate buffer sizes for compute and communication. (we need to include a figure, madeup). Standard MoE-block compute generally follows 2 strategies, one all-to-all and another all-gather. In all-to-all tokens are dispatched to topk experts spread across expert group (over ETP*EP, or EP groups for MoE-Folding(cite)). In All-to-All, split tokens are collected from (ETP*EP or EP groups in MoE-Folding(cite). As discussed earlier (motivation), this creates very large intermediate buffers (activations*topk*4). These large preparatory buffers, and post-processing buffers are unavoidable as long as the communication pattern is either all-to-all or all-gather. In Ring-MoE, rather than having one single step all-to-all for topk dispatch, expert compute, and then another all-to-all for combining outputs, we compute in MoE block in a rotating stream among the experts (later section). This design can allow much greater memory efficiency, which is impossible with all-to-all or all-gather. Ring-MoE design depends on moving experts or token activations with adaptive choices for optimal communication pattern. We follow a localized compute pattern that computes parts that are locally placed in a GPU. In any compute and communication pattern, the input activation and the final output activation size remain the same. In all-to-all/all-gather variation, the routing-map is used to get the top-k experts for all the local tokens in a rank, and then the buffer creation happens for dispatch. But this dispatch includes all the experts in that layer spread across ep-communication group because a single token can select any expert (placed in local or remote rank). So, this global dispatching is what causing buffer creation for sending, receiving, and reorganizing to prepare for GEMM. The GEMM could either be grouped or sequential for local experts only happening in different ranks with different experts concurrently. Ring-MoE avoids using a single dispatch or combine for the necessary communication. It uses the input token activations, routing-map, and experts and decides what part of the full expert computation can be computed locally in the Ring-MoE streaming pipeline. Then, it procceds to compute that partial computation for the full MoE required computation, and then moves the token-activations or expert weights and gradients in the expert-communication groups (section ..). This, totally removes the required top-k scaled intermediate buffers for dispatch, and combine for MoE-block, keeping the computation identical.  This includes the top-k scaled (permutation, dispatch all-to-all, post-process, combine all-to-all, and unpermutation). This keeps the memory requirement to input tensors, intermediate compute tensors, and only output tensors to its close to the activation sizes without top-k scling. At the same time, removing the top-k scaled communication buffers for all-to-all or all-gather as all communications are now peer-to-peer. In the following section, we discuss how we work with our adaptive routing algorithm for efficient communication.

additional section..\\

**notes: we keep whatever token we get from attention part per rank, and also whatever routing\_map we get from attention. Move only the experts. then see if a token has selected any current expert local to current GPU, if so, do the computation, otherwise skip it. So, we are not moving the routing\_map either.\\

\subsection{Adaptive Routing for Optimal Communication}
\begin{itemize}
    \item design of memory efficiency, \\
    \begin{itemize}
        \item expert-routing
        \item token-routing
    \end{itemize}
\end{itemize}
in the following sections, we provide a strategy to choose an option between routing experts or routing tokens.\\

\textbf{Ring-expert.} For expert routing cost can be approximated by the following.

\begin{align}
C_{of}, C_{ob} &=\frac{(N-1)EW}{B_e}\\
T_{\mathrm{expert}}
& \approx
\max\!\left(
C_{of},
T_{\mathrm{f}}
\right)
+\max\!\left(
C_{ob},
T_{\mathrm{b}}
\right)
+\frac{NEW}{B_e}
\end{align}

Where $W$ is single expert size, $E$ experts per GPU. $(N-1)$ comes from the number of hops required for moving expert weight buffer for forward and backward. We also have to move the expert gradients $(N)$ times in backward to put it into its original GPU rank. $C_{of}, C_{ob}$ are the overlapped expert buffer movement time. $B_{e}$ is the communication bandwidth. %$\alpha_e$ is the overhead.
$T_{f}$ and $T_{b}$ are the computation time for forward and backward which would be overlapped by routing the expert weights. These should be mostly overlapped(we can analyze in nsys to see if that is true.). We can further simplify this to communication only consideration for approximation:

\begin{align}
T_{\mathrm{expert}} &\approx  \frac{(3N-2)EW}{B_e}
\end{align}

\textbf{Ring-token.}
For routing tokens, we have to move the token activations, the intermediate activations after local expert computations. Along with that, we also required to move routing-map, and probability matrix, which are fixed cost. 

\begin{align}
C_{oft}, C_{obt}&=\frac{(N-1)(2T+R+P)}{B_{t}}\\
T_{\mathrm{token}}
\approx
&\max\!\left(
C_{oft},
T_{\mathrm{f}}
\right)
+\max\!\left(
C_{obt},
T_{\mathrm{b}}
\right)
+\frac{N(T+P)}{B_t}
\end{align}
Here, $T$ is the token activation size. In forward, and backward we need to move token activations, their intermediate activations after computing with experts. These $2T$ activations are moved $(N-1)$ hops both for forward, and backward in overlap with computation. Additionally, routing-map sized $R$, and routing probabilities $P$ are also moved. Assuming communication time will dominate, this can be simplified to the following:
\begin{align}
T_{\mathrm{token}} &\approx \frac{N(5T+2R+3P)}{B_t}
\end{align}
if $T_{token}>T_{expert}$, Ring-MoE prefers to route experts, rather than tokens for the best possible runtime performance. This is generally what happens, when we are training with reasonably long sequences. The communication remains static for expert-routing, which is not the case for token routing.\\


Static communication volume,... (algo.. with overlap..)..instead of .... at each stage ..hardware agnostic... as a result, Ring-MoE ...communications we avoid ... communications that we add. .. (forward: comm overlap ..., backward: expert overlap, gradients sequential ...) reduced P2P calls..., coalesced memory access ...inter-node bandwidth friendly...
how we maintain the indexing correct... how the activations are mapped back.. the processes (1)..(2)..(3)..(4)..(5).. from figure ...which buffers are replaced ... why .. and for what...refer to algo...p2p buffer construction...redundancy removal...\\

\subsection{Streaming Computation for Improved Scalability} 
a device compute outputs using the current set of expert weights while simultaneously preparing to exchange weights with neighboring devices. This enables a predictable and scalable communication pattern based only on nearest-neighbor transfers, which is often more efficient than global collectives... recompute friendly design...

\subsection{Asynchronous Triple Ring Orchestration}
in ring network, 3 rings are moved (compute, weight prefetch, accumulation of backward gradients)


\subsection{Load-balanced Zero-Drop Pipeline} (X-MoE is padding free, RingX talks about load balancing)
removes extra compute, padding, load balanced routing ... put some figure to explain with..stages...how forward+backward does not require any additional padding...why padding free..redundancy removal...
    \item token routing

%\subsection{Shared Experts Memory Reduction via Ring}
%have not implemented. we can reduce the shared expert load that happens per gpu. We will not include it.


\subsection{Recompute Friendly Backward Design}
    (4 page)
\end{itemize}
    

added figure here.




\section{Implementation}
ring-algorithm


==> text/eval.tex <==
\section{Evaluation}

\subsection{Experimental Setup \textcolor{blue}{updated}}
\label{sec:setup}
\paragraph{Platform}
All experiments were run on MareNostrum~5 in the Accelerated (ACC) partition. Each node contains four NVIDIA H100 GPUs (64\,GB HBM2e per GPU) and two Intel Xeon Platinum 8460Y+ CPUs (40 cores each). GPUs within a node are interconnected via NVLink~4.0, and nodes are connected through an NDR InfiniBand network with a fat-tree topology~\cite{MN5}. 


\paragraph{Models} 


 We evaluate \name in two complementary settings, summarized in Table~\ref{tab:models}. First, to measure end-to-end benefits under realistic pretraining workloads, we use three production MoE architectures: Qwen2-57B-A14B, Qwen3-30B-A3B, and Qwen3.5-35B-A3  (Table~\ref{tab:models}). The three span the design space along the dimensions that matter for MoE dispatch: Qwen2-57B combines shared and routed experts with a wide expert FFN, Qwen3-30B uses fine-grained routed experts, and Qwen3.5-35B doubles the expert count with a narrower expert FFN and a hybrid attention design. Unless otherwise noted, all end-to-end experiments use 8 nodes(32 GPUs) with TP=2, CP=4, PP=4, and EP=8. Second, to isolate how MoE design choices affect memory and throughput under \name, we construct Qwen3-style scaling configurations that vary the number of experts (64--384), the routing degree (top-4 to top-16), and the expert FFN width (512--2048). These experiments use 2 nodes (8 GPUs) with TP=4, CP=2, PP=1, and EP=8. We adjust the number of layers to keep the total trainable parameter count comparable across settings. In all experiments, we enable NVIDIA's MoE Parallel Folding \cite{moeparallelfolding2025}, which allows attention and MoE layers to use flexible and independent parallelism configurations. Furthermore, we compare scaling performance with the same models but with MoE-only variants.
 
 %\textcolor{red}{did Jaume used TP=2,CP=4? because for 2-node experiments we used TP=4, CP=2. We need to mention that for GQAttention, we did not use a sliding window; if we did, the attention should be much faster, require less memory, and our MoE gain should be higher.}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/eval/ATC_qwen3_qwen35_qwen2.pdf}
    %\vspace{-5pt}
    \caption{End-to-end training throughput on production MoE architectures. (a) Qwen3-30B-A3B and (b) Qwen3.5-35B-A3B: \name is faster at every tested sequence length and trains at up to 786K tokens, where all-to-all runs out of memory. (c) Qwen2-57B-A14B:all-to-all runs out of memory even at 393K, while \name trains it.}
    \label{fig:overall_perf}
    %\vspace{-10pt}
\end{figure*}

\input figures/table_models

\paragraph{Software and baselines \textcolor{blue}{updated}}

We implement \name on top of Megatron-LM~\cite{megatron-lm} in 2.3K lines of code. Our primary baseline for end-to-end model training is the default all-to-all MoE dispatcher of the latest Megatron-LM release (May 2026), which follows the standard dispatch-then-compute execution model. We also enable DeepEP~\cite{deepep2025} within Megatron-LM, which optimizes token dispatch and combine while retaining the same all-to-all formulation. We evaluate DeepEP only with intra-node expert parallelism (EP$=$4), because cross-node DeepEP requires InfiniBand GPU Direct Async (IBGDA), which depends on NVSHMEM and NIC configurations that are not available on our platform; the all-to-all baseline and \name use EP$=$8 across two nodes. All three systems share the same model architecture, parallelism configuration, and training hyperparameters. We report training throughput in TFLOPS per GPU, excluding recomputation FLOPs. \textcolor{blue}{For MoE-only scaling  comparison, \name is compared against Megatron-LM all-to-all,  Tutel ~\cite{tutel}, and FasterMoE ~\cite{fastermoe2022}. For scaling comparison, everything was fully in GPU without any offloading or recomputation.}


\subsection{End-to-End Performance on a Production Model \textcolor{blue}{updated}}
%We begin by evaluating \name on a realistic pretraining workload. Figure~\ref{fig:overall_perf} shows training throughput on Qwen3-30B-A3B and Qwen2-35B-A3B across varying sequence lengths. At each sequence length, we select the largest micro-batch size to fully utilize all available GPU memory. 
%On Qwen3-30B, \name achieves higher throughput than the all-to-all baseline by up to 21.7\% at every sequence length since its reduced peak memory allows larger batch sizes. Beyond 393K, the all-to-all baseline runs out of memory regardless of batch size, while \name continues to train up to 786K tokens, a 2$\times$ improvement in maximum trainable sequence length.
%On Qwen3.5-35B, the larger expert dimension and different expert FFN size, we get similar throughput benefits for similar experiments. This model successfully trains context of 786k also, enabling a training setting that is otherwise impossible under the same hardware budget with alltoall.
%The following scaling experiments analyze the mechanisms behind these gains in more controlled settings.

We first evaluate \name on realistic pretraining workloads. Figure~\ref{fig:overall_perf} shows training throughput on Qwen3-30B-A3B, Qwen3.5-35B-A3B, and Qwen2-57B-A14B across varying sequence lengths. At each sequence length, we select the largest micro-batch size to fully utilize all available GPU memory. 
On both Qwen3-30B and Qwen3.5-35B, \name achieves higher throughput than the all-to-all baseline at every sequence length, by up to \textcolor{blue}{26\%}, since its reduced peak memory allows larger batch sizes. Beyond 393K, all-to-all runs out of memory regardless of batch size, while \name continues to train up to 786K tokens, a 2$\times$ improvement in maximum trainable sequence length. The gains hold despite the two models differing in expert granularity: Qwen3.5-35B doubles the expert count with a narrower expert FFN. On Qwen2-57B, the larger hidden dimension and wider expert FFN amplify every dispatch buffer further: all-to-all runs out of memory even at 393K, while \name trains this configuration. The following scaling experiments analyze the mechanisms behind these gains in more controlled settings.


\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/eval/ATC_seqlen_scaling_merged_ring.pdf}
    %\vspace{-10pt}
    \caption{Sequence length scaling study across model configurations with fixed micro-batch size ($b=12$) and full activation recomputation. \name consistently supports longer trainable sequence lengths than all-to-all. (updated after ATC)}
    \label{fig:eval_seq}
\end{figure*}
% \textcolor{red}{updated}

\subsection{Sequence Scaling for Longer Context and Higher Throughput \textcolor{blue}{updated.}}
In this section, we evaluate how \name converts its lower MoE memory footprint into longer trainable context. Using the same 8-GPU scaling-study setup, we fix the micro-batch size to $b=12$ for both dispatchers and increase the training sequence length until reaching the GPU memory limit. 

Figure~\ref{fig:eval_seq} reports the resulting throughput at each feasible sequence length. Overall, \name provides two benefits simultaneously: it expands the trainable context window and converts that larger feasible context into higher training throughput.
First, \name substantially increases the maximum trainable sequence length. All configurations run at sequence length 40K with both dispatchers. As the context length increases, all-to-all quickly becomes memory-limited: at 65K, the \texttt{E64}, \texttt{K12}, and \texttt{K16} configurations already run out of memory, and no configuration except \texttt{K4} trains beyond 65K with all-to-all. In contrast, \name runs all models at 65K and extends the maximum trainable context to 90K--150K, depending on configuration, increasing the maximum trainable sequence length by up to 2.85$\times$ over all-to-all.
% 114/40=2.85

Second, the additional context also improves throughput. Throughput increases as sequence length grows, since the larger per-step workload better amortizes fixed overheads and raises hardware utilization. All-to-all is not runable in this case due to the memory limit at shorter sequence lengths. As a result, \name not only enables longer-context training, but also achieves higher throughput by operating efficiently that is inaccessible to the all-to-all baseline.


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/eval/ATC_merged_ring_recompute_scaling_study.pdf}
    %\vspace{-10pt}
    \caption{Training throughput benefit obtained by reducing the number of recomputed layers across model configurations at three long-context settings (40960, 65536, and 98304 tokens).} % fused ring, on 29 August
    %\vspace{-5pt}
    \label{fig:recompute_scal}
\end{figure*}
%\textcolor{red}{updated}
\subsection{Recompute Reduction for Improved Throughput. \textcolor{blue}{updated}}
We evaluate whether the memory savings of \name can be translated into higher pretraining throughput by reducing activation recomputation. We use the scaling configurations from Table~\ref{tab:models} and evaluate three long-context settings with sequence lengths 40K, 65K, and 98K. For these three sequence lengths, we use micro-batch sizes 12, 8, and 5, respectively, which keeps the number of tokens per step approximately constant. For each model configuration and each dispatcher, we progressively reduce the number of recomputed layers and select the smallest value that still fits in GPU memory.

%Figure~\ref{fig:recompute_scal} shows that the lower peak memory of \name consistently translates into a less aggressive checkpointing schedule and therefore higher throughput. In most configurations, \name outperforms the all-to-all baseline, with speedups reaching up to 1.73$\times$. The gains are most pronounced in the more memory-constrained scenarios, where the all-to-all baseline requires substantial recomputation to fit, while \name can run with fewer or no recomputed layers. This result validates \name adaptively reduces activation checkpointing and converts the recovered memory budget into throughput gains by avoiding redundant recomputation. In contrast, the few cases where all-to-all remains competitive or slightly faster correspond to configurations that already fit with little or no recomputation, with \name operating significantly below the memory limit. In those cases, the recovered memory headroom is more naturally traded for larger batch size, longer context, or larger model capacity.

Figure~\ref{fig:recompute_scal} shows that the lower peak memory of \name consistently translates into a less aggressive checkpointing schedule and therefore higher throughput. In most configurations, \name outperforms the all-to-all baseline, with speedups reaching up to 2.02 $\times$. The gains are pronounced in memory-constrained scenarios, where the all-to-all baseline requires substantial recomputation to fit, while \name can run with fewer or no recomputed layers. This result validates \name adaptively reduces activation checkpointing and converts the recovered memory budget into throughput gains by avoiding redundant recomputation. In contrast, the few cases where all-to-all remains competitive or slightly faster correspond to configurations that already fit with little or no recomputation, with \name operating significantly below the memory limit. In those cases, the recovered memory headroom is more naturally traded for larger batch size, longer context, or larger model capacity.
% 2.02 for K16

\subsection{Batch Scaling for Improved Throughput. \textcolor{blue}{updated}} 
We evaluate the performance impact of micro-batch size at fixed sequence length. We use the same 8-GPU setup as in the scaling study, fix the sequence length to 40{,}960, and set the number of recomputed layers to the minimum non-OOM value required by the all-to-all baseline for each model. 

Figure~\ref{fig:batch_scaling} reports three settings for each configuration: all-to-all at micro-batch size $b{=}12$, \name at the same micro-batch size and \name at the largest micro-batch size that fits under the same sequence length and recomputation schedule. 

%% we show separately the performance gain for dispatchers.
%The middle bar therefore isolates the effect of the dispatcher itself, while the right bar shows how the recovered memory can be reinvested into larger training steps. \textcolor{red}{(ring b=12 is using full memory and diffrent recompute)}

At the same batch size, \name is already competitive and faster in most configurations. Across these configurations, \name reduces peak memory by up to 35.7\% relative to all-to-all. This allows scaling the micro-batch size substantially, from 12 up to 40 depending on the model. The larger step size translates into higher throughput, yielding an average speedup of 1.42$\times$ over all-to-all. These results show that even when ring-based dispatch does not provide a throughput advantage over default all-to-all, the recovered memory can still be converted into end-to-end speed by increasing the amount of work processed per step.
%(2) fix seq length \& fix recompute , batch size: expect to see training throughput (significant)  improvement

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/eval/ATC_batch_scaling_merged_ring.pdf}
    %\vspace{-15pt}
    \caption{Training throughput across model configurations at 40{,}960 sequence length. Bars show all-to-all at micro-batch size $b=12$, \name at the same batch size, and \name at the largest micro-batch size that fits under the same sequence length and recomputation schedule (annotated numbers).(updated 29 August, the b=12 has a different recompute layers to fill GPU for ring)} % updated after ATC
    %\vspace{-10pt}
    \label{fig:batch_scaling}
\end{figure}




\begin{comment}
\subsection{Comparison with DeepEP.}

We also compare \name against \textit{DeepEP}, a stronger all-to-all baseline that replaces the standard dispatcher with optimized MoE communication kernels. We evaluate all synthetic Qwen3-style configurations.  For this experiment, we set the expert-parallel degree to EP$=4$, so that the \textit{DeepEP} communication path remains intra-node on our system, which provides 4 H100 GPUs per node. Figure~\ref{fig:deepep} reports the resulting throughput across sequence lengths.

\textit{DeepEP} is slightly faster at the sequence lengths where both methods fit, reflecting the efficiency of its hardware-specialized all-to-all kernels. However, its feasible context range is smaller. \textit{DeepEP} cannot run at sequence length 98K, while \name remains trainable. This is because \textit{DeepEP} improves the efficiency of all-to-all dispatch, but it does not change the underlying dispatch-then-compute execution model. As a result, it does not eliminate the top-k-expanded MoE activation buffers that dominate peak memory in long-context training.  Overall, these results show that while \textit{DeepEP} can be a very strong baseline when the all-to-all formulation still fits comfortably, \name is substantially more robust in the memory-constrained long-context regime. 

A second difference is portability. \textit{DeepEP} is tightly coupled to NVIDIA-specific communication mechanisms. Its implementation relies on NVLink for intra-node communication and on RDMA, NVSHMEM, and InfiniBand GPU Direct Async (IBGDA) for efficient inter-node execution, together with correct GPU-NIC affinity. On our cluster, which provides only 4 H100 GPUs per node, any configuration with EP$>4$ necessarily requires this inter-node communication path. However, in our current environment, inter-node \textit{DeepEP} is not functional. In contrast, \name does not depend on specific kernels or a specialized communication stack. As a result, \name is less tied to a particular hardware and software environment, while still delivering substantially better scalability in the long-context regime.
\end{comment}



\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/eval/adaptive_routing_comparison.pdf}
    %\vspace{-10pt}
    \caption{Adaptive routing comparison on large-expert configurations where expert transfer can dominate communication volume.}
    %\vspace{-20pt}
    \label{fig:adaptive_routing}
\end{figure}


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/eval/ATC_baseline_comparison_seqlen.pdf}
    %\vspace{-15pt}
    \caption{RingMoE MoE only latency comparison with Megatron-AlltoAll, Tutel, and FasterMoE for EP=8 with 8 GPUs}
    %\vspace{-5pt}
    \label{fig:baseline_seq_scaling}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/eval/ep_scaling_ring_vs_alltoall_vs_tutel_vs_fastermoe.pdf}
    %\vspace{-15pt}
    \caption{RingMoE scales much better compared to Megatron all-to-all, Tutel, and FasterMoE over EP=8 to 64 for MoE-only latency comparison, where each rank possesses the same amount of tokens. For \texttt{K12} and \texttt{K16} Tutel can not run.}
    %\vspace{-5pt}
    \label{fig:baseline_ep_scaling}
\end{figure*}

\subsection{Micro-Optimization Ablation Study \textcolor{blue}{updated}}

% the following paragraph was in ATC submission.

%To quantify the contribution of \name's overlap optimizations, we measure forward and backward pass time on Qwen3-30B-A3B under three configurations: O1 (no overlap), O2 (weight prefetch overlapped with computation), and O3 (weight prefetch and weight gradient transfer both overlapped, implementing the full triple-ring orchestration from Section~\ref{sec:overlap}). Figure~\ref{fig:overlap_ablation} decomposes each configuration into overlapped and non-overlapped portions.
%In the forward pass, O2 reduces runtime from 98.6 ms to 71.9 ms (27\% reduction) by overlapping expert weight prefetch with local computation at each hop. In the backward pass, O2 reduces runtime from 266.6 ms to 186.8 ms (30\% reduction). O3 further reduces the backward pass from 186.8 ms to 171.3 ms by additionally overlapping weight gradient transfer through in-place addition (Section~\ref{sec:overlap}). In total, the triple-ring orchestration achieves a 35\% reduction in forward time and 36\% reduction in backward time compared to no overlap.

% the following is for Eurosys submission, the above was for ATC and ASPLOS submission.

To quantify the contribution of \name's optimizations, we show forward and backward pass time for the \texttt{E128} MoE-only model running fully in GPU with EP=8 as an example, with fixed token counts, everything in GPU. In Figure ~\ref{fig:overlap_ablation}, the first bar shows vanilla RingMoE with compute and communication non-overlapped, taking 295.9 ms per single iteration. For \name with weight and gradient overlap in the second bar, we combine the weights, and gradients in single tensor payload and move while the compute is ongoing at each hop for full overlap. This  reduces the forward pass time from 89.46 to 50.76 ms, and backward pass from 206.39 to 143.67 ms. This improves the total latency by 31.2$\%$ compared to vanilla \name. Finally, we also include incorporation of \texttt{GroupedGEMM} both in forward and in backward pass, reducing the total latency to 175.8 ms. \name can incorporate other optimized GEMM kernels also, we show \texttt{GroupedGEMM} as an example. 

\subsection{Token Scaling Performance \textcolor{blue}{updated}}
We compare  MoE-only performance against Megatron all-to-all, Tutel, and FasterMoE.  Single SwiGLU MoE-only models are created from the same config as Table ~\ref{tab:models}.  \texttt{E128/H768/K8} becomes the same model.  In Figure ~\ref{fig:baseline_seq_scaling}, for batch=12, we increase total seqlen from 40K to 98K, but keep the GPU count the same. RingMoE on average is 2$\times$ faster than all-to-all.  For a similar SwiGLU layer config such as \texttt{E128} matching  Qwen3-30B-A3B, the speedup is 1.76--2.4$\times$ faster than all-to-all. For models such as \texttt{E384, H2048}, where \name is slightly slower, end-to-end models could increase batch sizes to gain more performance. Compared to FasterMoE, \name is on average 4.02$\times$ faster, with speedups ranging from 1.41 to 6.19$\times$. \name is 2.63$\times$ faster on average compared to TUTEL. TUTEL cannot run models \texttt{E64, E128, E384, K12, K16, H512, H2048} often for 65K and 98K seqlens.  %For Models, like \texttt{E384, H2048} where RingMoE is slower, we have shown we can increase batch 

\subsection{EP Scaling Performance \textcolor{blue}{updated}}
Figure ~\ref{fig:baseline_ep_scaling} compares the same MoE-only layer baselines across expert-parallelism (EP) degrees of 8, 16, 32, and 64, with batch size=12 and per-rank sequence length=8192. \name consistently achieves the lowest and fastest latency across all the combinations. \name also provides the lowest growth factor among baselines, ranging from 1.12 to 1.68$\times$ for various models when scaled from EP=8 to 64. Megatron all-to-all is slower in latency compared to \name and grows by 1.5 to 2.25$\times$ with EP scaling across models. TUTEL is slower than both and did not run on models with larger top-k such as \texttt{K12, K16}. FasterMoE ran for all the models, but was the slowest in latency among all the baselines, with a growth ranging from 2.1 to 7.2$\times$ across models. \name scales better than others due to the reduced amount of communication volume. \name also reduces memory usage. At EP=8, \name reduces peak memory usage ranging from 2.6 $\times$ (E384) to 5.1$\times$  (K16), averaging 3.8$\times$  across the eight configurations. By EP=32, the average peak memory use reduction grows to 7.3$\times$  (2.6$\times$ –11.8$\times$ ), and at EP=64 it reaches 7.6$\times$ on average, peaking at 10.2$\times$ for K12 and 13.4$\times$  for K16.

%for ep=16, e64: ring:1208mb and alltoall: 6380mb
%e128: ring:1471mb and alltoall: 6400mb
%e384: 


%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{figures/eval/overlap_breakdown.pdf}
%    %\vspace{-5pt}
%    \caption{Forward and backward runtime breakdown for Qwen3-30B-A3B under three overlap configurations: O1 (no overlap), O2 (overlapping expert weight prefetch with computation), and O3 (full triple-ring overlap, additionally overlapping weight-gradient transfer (update-redesign)).}
     %\vspace{-20pt}
%    \label{fig:overlap_ablation}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/eval/Eurosys_micro_opt_ablation.pdf}
    %\vspace{-5pt}
    \caption{RingMoE latency improves by overlapping expert and gradient transfer with compute. GroupedGEMM further improves the latency. (W. \& G. = weight \& gradient) }
     %\vspace{-20pt}
    \label{fig:overlap_ablation}
\end{figure}


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/eval/ATC_deepEP.pdf}
    %\vspace{-15pt}
    \caption{\name comparison with DeepEP across  scaling-study configurations (Table~\ref{tab:models}) with intra-node expert parallelism (EP$=$4).}
    %\vspace{-5pt}
    \label{fig:deepep}
\end{figure*}


\subsection{Comparison with DeepEP \textcolor{blue}{updated}}


We compare \name against DeepEP, an all-to-all baseline with optimized communication kernels, on all ten scaling-study configurations (Table~\ref{tab:models}) at sequence lengths 40K, 65K, and 98K, with EP$=$4 so that the DeepEP communication path remains intra-node on our platform (\S\ref{sec:setup}). We ran DeepEP with a fixed batch size, but with the lowest possible recompute so that peak memory is used to get the maximum possible throughput. For \name, we kept the recompute count the same as DeepEP but increased the batch size. Figure~\ref{fig:deepep} reports the results.

When both dispatchers fit in memory, their throughput is comparable. However, DeepEP ran out of memory on several models at 98K context (\texttt{K8}, \texttt{K12}, \texttt{K16}, and \texttt{H512}). Model \texttt{H2048}, is slower for \name because of very large weights, routing involves substantially more data movement, and DeepEP's highly optimized communication kernels for this kind of hardware, delivers slightly better performance.

%At 40K, the two differ by at most 7\%, and the difference remains limited at 65K and 98K wherever DeepEP still fits. As training sequence length increases, however, DeepEP quickly reaches the memory limit: at 98K it trains only 2 of the 10 models, while \name trains 8, failing only on E64 and H512, whose depth-heavy designs are memory-bound outside the MoE block (Table~\ref{tab:models}).
DeepEP itself depends on a specialized communication stack, NVSHMEM and IBGDA with correct GPU--NIC affinity, for inter-node execution, which we could not enable on our platform and which restricts it to EP$\le$4 in our setup (\S\ref{sec:setup}); \name needs only
point-to-point transfers and runs across nodes unmodified. Overall, \name matches DeepEP where all-to-all fits and trains where it cannot, with a memory bound that holds at every iteration.

The deeper limitation for any variant of all-to-all dispatch is that it forces a choice between memory safety and model quality. When running with drop-less tokens or limited token-drop, the buffers are sized by the routed load, so peak memory varies across iterations and spikes under routing imbalance, which is most severe in early training~\cite{memfine2025}; a configuration that fits on average can still fail mid-run. The alternative bounds memory with a capacity factor, dropping the tokens that exceed each expert's capacity at a cost in model quality~\cite{moeparallelfolding2025}.
DeepEP accelerates both modes with specific hardware, but escapes neither of the issues. \name removes the dilemma: it is drop-less, and the ring schedule fixes its peak memory constant across iterations and independent of routing decisions.



\subsection{Adaptive Routing: Token vs Expert \textcolor{blue}{updated}}
To validate \name's adaptive routing, we use two configurations, \texttt{MoE-E384-K12} and \texttt{MoE-E384-K16}, both with 384 experts, top-$k$ values of 12 and 16 respectively, hidden dimension 2048, and expert FFN width 2048 (19.53B parameters total). The combination of many experts per GPU and wide FFN makes expert routing transfer large volumes of expert weights at each hop.

Figure~\ref{fig:adaptive_routing} compares\name with all-to-all. On \texttt{MoE-E384-K12}, token routing achieves 3.7$\times$ higher throughput than expert routing at 20K (58.3 vs.\ 15.9 TFLOPs/GPU) and 2.1$\times$ at 40K (89 vs.\ 42 TFLOPs/GPU). Even the all-to-all baseline (included for reference at 20K) is outperformed by token routing. On \texttt{MoE-E384-K16}, token routing similarly outperforms expert routing across sequence lengths. These results confirm that expert routing is not universally optimal: when expert weights per GPU exceed token activations, token routing yields significantly better throughput. \name's cost model (\S~\ref{sec:adaptive}) selects the correct mode from model configuration and parallelism settings without manual tuning.


\subsection{Training Correctness \textcolor{blue}{updated}}
We verify \name preserves training correctness relative to the standard all-to-all dispatcher by training Qwen3-30B-A3B with \name and all-to-all using the same initialization, random seed, and training hyperparameters. Figure~\ref{fig:loss} shows that the two loss curves are indistinguishable over 1500 training iterations. This is consistent with the mathematical equivalence of the two formulations (Section~\ref{sec:local}): the only expected deviation is floating-point rounding from the different accumulation order, which has no impact on convergence.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/eval/lm_loss_comparison.pdf}
    %\vspace{-20pt}
    \caption{Training loss for Qwen3-30B-A3B using \name and all-to-all dispatch under identical initialization and hyperparameters. }
     %\vspace{-10pt}
    \label{fig:loss}
\end{figure}

